Volume-Centred Range Bars: Novel Interpretable Representation of Financial Markets Designed for Machine Learning Applications

Financial markets are a source of non-stationary multidimensional time series which has been drawing attention for decades. Each financial instrument has its specific changing-over-time properties, making its analysis a complex task. Hence, improvement of understanding and development of more informative, generalisable market representations are essential for the successful operation in financial markets, including risk assessment, diversification, trading, and order execution. In this study, we propose a volume-price-based market representation for making financial time series more suitable for machine learning pipelines. We use a statistical approach for evaluating the representation. Through the research questions, we investigate, i) whether the proposed representation allows the more efficient design of machine learning models; ii) whether the proposed representation leads to increased performance over the price levels market pattern; iii) whether the proposed representation performs better on the liquid markets, and iv) whether SHAP feature interactions are reliable to be used in the considered setting. Our analysis shows that the proposed volume-based method allows successful classification of the financial time series patterns, and also leads to better classification performance than the price levels-based method, excelling specifically on more liquid financial instruments. Finally, we propose an approach for obtaining feature interactions directly from tree-based models and compare the outcomes to those of the SHAP method. This results in the significant similarity between the two methods, hence we claim that SHAP feature interactions are reliable to be used in the setting of financial markets.

==> README <==
Permission is granted to copy, distribute and/or modify this software under
the terms of the LaTeX Project Public License, version
1.3c (http://www.latex-project.org/lppl.txt). The current
maintainer is Philip Kime (© 2019).

This package is a biblatex style for APA (American Psychological
Association) style compliant documents typeset in LaTeX. It
implements a citation style (apa.cbx) and a references section style
(apa.bbx). The styles are loaded just like any other biblatex
styles but I wouldn't try to use the citation and references styles
separately as they rely on each other, macro-wise, in places.

In this document and in the code, the specific APA requirements are
referred to by the section and (if appropriate) the example number of the
APA Style Guide 7th Edition).

You will need to be using csquotes >= 4.3 and biblatex >= 3.4 The biber
backend for biblatex >= 2.5 is also required. This style will not work
correctly if using bibtex as the backend for biblatex. If you want to take
advantage of the biblatex \DeclareQuotePunctuation facility to enforce the
APA required "American punctuation", you should use the babel package with
the "american" option (see biblatex manual section |3.9.1|). You can of
course use other languages but in such cases, to adhere to APA "American"
punctuation rules (following commas moved inside closing quotes etc.), then
you should set up \DeclareQuotePunctuation yourself as per section 4.7.5 of
the biblatex manual.

You can also use this with apa.cls version 1.3.4 or greater by using the 
"noapacite" class option to that class package (which prevents it from
trying to use plain bibtex with the apacite package).

Please refer first to biblatex-apa.pdf for the main documentation.



